Cardea: An Open Automated Machine Learning Framework for Electronic Health Records

An estimated 180 papers focusing on deep learning and EHR were published between 2010 and 2018. Despite the common workflow structure appearing in these publications, no trusted and verified software framework exists, forcing researchers to arduously repeat previous work. In this paper, we propose Cardea, an extensible open-source automated machine learning framework encapsulating common prediction problems in the health domain and allows users to build predictive models with their own data. This system relies on two components: Fast Healthcare Interoperability Resources (FHIR) -- a standardized data structure for electronic health systems -- and several AUTOML frameworks for automated feature engineering, model selection, and tuning. We augment these components with an adaptive data assembler and comprehensive data- and model- auditing capabilities. We demonstrate our framework via 5 prediction tasks on MIMIC-III and Kaggle datasets, which highlight Cardea's human competitiveness, flexibility in problem definition, extensive feature generation capability, adaptable automatic data assembler, and its usability.

==> tables/tasks.tex <==
\begin{table}
  \centering
  \setlength{\extrarowheight}{0pt}
  \addtolength{\extrarowheight}{\aboverulesep}
  \addtolength{\extrarowheight}{\belowrulesep}
  \setlength{\aboverulesep}{0pt}
  \setlength{\belowrulesep}{0pt}
  \caption{Experimental tasks.}
  \label{tab:tasks}
  \begin{tabular}{l!{\vrule width \lightrulewidth}p{7.5cm}} 
  \toprule
  Task                                 & Question                                                                                                        \\ 
  \midrule
  \rowcolor[rgb]{0.933,0.933,0.933} T1 & \textcolor[rgb]{0.122,0.122,0.141}{Q1. How many entries were in the \`{}icustays\`{} table?}                    \\
                                       & Q2. Is it helpful to display the "relationship" of the entityset?                                               \\ 
  \midrule
  \rowcolor[rgb]{0.933,0.933,0.933} T2 & \textcolor[rgb]{0.122,0.122,0.141}{Q3. Given the data, can we predict a patient's ICU time?} \\
                                       & \textcolor[rgb]{0.122,0.122,0.141}{Q4. Given the data, what is your prediction problem?}                        \\
  \rowcolor[rgb]{0.933,0.933,0.933}    & \textcolor[rgb]{0.122,0.122,0.141}{Q5. Does your prediction problem already exist in Cardea?}                   \\ 
  \midrule
  T3                                   & \textcolor[rgb]{0.122,0.122,0.141}{Q6. How many features were generated?}                                       \\
  \rowcolor[rgb]{0.933,0.933,0.933}    & \textcolor[rgb]{0.122,0.122,0.141}{Q7. What is the datatype of y?}                                              \\ 
  \midrule
  T4                                   & \textcolor[rgb]{0.122,0.122,0.141}{Q8. Can you get a model with accuracy \textgreater{} 80\%?}          \\
  \rowcolor[rgb]{0.933,0.933,0.933}    & Q9. What was the best accuracy score you obtained?                                                                  \\
  \bottomrule
  \end{tabular}
  \end{table}

==> tables/tasks_data.tex <==
\begin{table}
  \centering
  \setlength{\extrarowheight}{0pt}
  \addtolength{\extrarowheight}{\aboverulesep}
  \addtolength{\extrarowheight}{\belowrulesep}
  \setlength{\aboverulesep}{0pt}
  \setlength{\belowrulesep}{0pt}
  
  \begin{tabular}{c|c|ccc} 
  \toprule
  \multicolumn{1}{l|}{\textbf{Task}} & \multicolumn{1}{l|}{\textbf{Accuracy}}                    & \multicolumn{3}{c}{\textbf{Completion Time}}                    \\
                                     &                                                           & Cardea (min)         & Baseline (min)         & Times (x)       \\ 
  \cmidrule{1-2}\cmidrule(lr){3-3}\cmidrule(lr){4-4}\cmidrule(lr){5-5}
  T1                                 & Q1 100\%                                                  & 4.86 (2.25)          & 49.50 (52.70)          & 10.19           \\ 
  \midrule
  T2                                 & Q3 70\%                                                   & \textbf{5.77 (2.11)} & 32.00 (31.08)          & 5.55            \\ 
  \midrule
  T3                                 & \begin{tabular}[c]{@{}c@{}}Q6 80\%\\Q7 100\%\end{tabular} & 4.45 (0.84)          & \textbf{114.5 (69.94)} & \textbf{25.73}  \\ 
  \midrule
  T4                                 & Q8 100\%                                                  & 4.25 (3.77)          & 43.12 (37.58)          & 10.15           \\
  \bottomrule
  \end{tabular}
  \caption{Experimental results. Task time is shown in avg.(std.). The speed-up times of every task are reported.}
  \label{tab:tasks_data}
\end{table}
